Neural Parameter Search for Slimmer Fine-Tuned Models and Better Transfer

Foundation models and their checkpoints have significantly advanced deep learning, boosting performance across various applications. However, fine-tuned models often struggle outside their specific domains and exhibit considerable redundancy. Recent studies suggest that combining a pruned fine-tuned model with the original pre-trained model can mitigate forgetting, reduce interference when merging model parameters across tasks, and improve compression efficiency. In this context, developing an effective pruning strategy for fine-tuned models is crucial. Leveraging the advantages of the task vector mechanism, we preprocess fine-tuned models by calculating the differences between them and the original model. Recognizing that different task vector subspaces contribute variably to model performance, we introduce a novel method called Neural Parameter Search (NPS-Pruning) for slimming down fine-tuned models. This method enhances pruning efficiency by searching through neural parameters of task vectors within low-rank subspaces. Our method has three key applications: enhancing knowledge transfer through pairwise model interpolation, facilitating effective knowledge fusion via model merging, and enabling the deployment of compressed models that retain near-original performance while significantly reducing storage costs. Extensive experiments across vision, NLP, and multi-modal benchmarks demonstrate the effectiveness and robustness of our approach, resulting in substantial performance gains. The code is publicly available at: https://github.com/duguodong7/NPS-Pruning.

==> 8_Acknowledgement.tex <==
\section*{Acknowledgements}

% This work was supported in part by Shenzhen College Stability Support Plan (GXWD20231128103232001), Department of Science and Technology of Guangdong (2024A1515011540), Shenzhen Start-Up Research Funds~(HA11409065), National Natural Science Foundation of China (12204130), the Ministry of Higher Education Malaysia through the Fundamental Research Grant Scheme (FRGS/1/2023/ICT02/XMU/02/1), and Xiamen University Malaysia through Xiamen University Malaysia Research Fund (XMUMRF/2022-C10/IECE/0039 and XMUMRF/2024-C13/IECE/0049).


% This research is supported by the Ministry of Higher Education Malaysia through the Fundamental Research Grant Scheme (FRGS/1/2023/ICT02/XMU/02/1), and Xiamen University Malaysia through Xiamen University Malaysia Research Fund (XMUMRF/2022-C10/IECE/0039 and XMUMRF/2024-C13/IECE/0049).

==> files/checklist.tex <==
\appendix
% \section{Reproducibility Checklist}
% % \answerYes \answerNo \answerNA
%     % \answerNo{No, because}
% \begin{enumerate}



% \item This paper:
% \begin{enumerate}
%     \item  Includes a conceptual outline and/or pseudocode description of AI methods introduced? 
%     \answerYes{Yes, as shown in Section~\ref{sec:method}.}
%     \item  Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results? \answerYes{Yes, as shown in Section~\ref{sec:introduction}.}
%     \item  Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper? \answerYes{Yes}
% \end{enumerate}

% \item Does this paper make theoretical contributions? \\
% \answerNo{No, because this paper primarily focuses on machine learning applications in the areas of knowledge transfer and fusion.}

% \item Does this paper rely on one or more datasets? \answerYes{Yes}
% \begin{enumerate}
% \item A motivation is given for why the experiments are conducted on the selected datasets \answerYes{Yes}
% \item All novel datasets introduced in this paper are included in a data appendix. \answerYes{Yes}
% \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{Yes}
% \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. \answerYes{Yes}
% \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. \answerYes{Yes}
% \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. \answerYes{Yes}
% \end{enumerate}

% \item Does this paper include computational experiments? \answerYes{Yes}

% \begin{enumerate}
% \item Any code required for pre-processing data is included in the appendix. \answerYes{Yes}.
% \item All source code required for conducting and analyzing the experiments is included in a code appendix. \answerYes{Yes}
% \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. \answerYes{Yes}
% \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. \answerYes{Yes}
% \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. \answerYes{Yes}
% \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. \answerYes{Yes}
% \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. \answerYes{Yes}
% \item This paper states the number of algorithm runs used to compute each reported result. \answerYes{Yes}
% \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. \answerYes{Yes}
% \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). \answerYes{Yes}
% \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. \answerYes{Yes}
% \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. \answerYes{Yes}
% \end{enumerate}

\end{enumerate}


    % (yes/partial/no/NA)

==> files/checklist_template1.tex <==

\section{Paper Checklist}
% \answerYes \answerNo \answerNA
    % \answerNo{No, because}
\begin{enumerate}



\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, as shown in Section~\ref{sec:introduction}.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, as shown in Section~\ref{subsec:disad}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes}
  \item Did you discuss any potential misuse of your work?
    \answerYes{Yes}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{Answer}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{Answer}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{Answer}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{Answer}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{Answer}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{Answer}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerTODO{Answer}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerTODO{Answer}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{Answer}
  \item Did you mention the license of the assets?
    \answerTODO{Answer}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerTODO{Answer}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{Answer}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{Answer}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
\answerTODO{Answer}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 
\answerTODO{Answer}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerTODO{Answer}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerTODO{Answer}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{Answer}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerTODO{Answer}
\end{enumerate}

\end{enumerate}

